High regularity waves on self-similar naked singularity interiors: decay and the role of blue-shift

We consider solutions to the linear wave equation $\Box_{g}\varphi = 0$ on a class of approximately $k$-self-similar naked singularity interiors. This equation models the blue-shift effect, an instability exploited by Christodoulou in the proof of low-regularity weak cosmic censorship. Using a combination of resonance expansions and multiplier estimates, we find in the small-mass regime $k^2 \ll 1$ that the asymptotics of solutions are strongly sensitive to the regularity assumed on outgoing, characteristic initial data across the past light-cone of the singularity. Above a threshold regularity set by the $k$-self-similar scalar field, solutions are shown to always obey self-similar bounds, indicating that the blue-shift instability competes with the stabilizing influence of high regularity. We conclude that a proper statement of weak cosmic censorship, as well as an understanding of the role of naked singularities in phenomena such as critical collapse, may depend on the topology of initial data.

==> replacealls.tex <==
To simplify the number of cases handled in the proof, assume that $\omega > 0$. The case $\omega = 0$ introduces additional boundary terms that are easily handled.
     
    Multiplying (\ref{eq:wavesim_alpha_comm1}) by $|z|^{2\omega}\br{r}^{-4}\partial_z \psi^{(1)}_\rho$ and integrating by parts in $\mathcal{R}(s_0)$ yields
    \begin{align}
        \frac{1}{2}\int_{\{s=s_0\}}&\frac{|z|^{2\omega}}{\br{r}^4}(\partial_z \psi^{(1)}_\rho)^2 + \frac{1}{2}\int_{\Gamma_{s_0}} \frac{\big(\partial_z \psi_\rho^{(1)} \big)^2 }{\br{r}^4} \nonumber \\[2\jot]
        +\iint_{\mathcal{R}(s_0)} &\big(\frac12 q_k(1-2\omega) + \rho + q_k |z| \partial_z \log w - \partial_s \log w \big) \frac{|z|^{2\omega}}{\br{r}^4}(\partial_z \psi^{(1)}_\rho)^2   \nonumber\\[2\jot]
        &= \frac{1}{2}\int_{\{s=0\}}\frac{|z|^{2\omega}}{\br{r}^4}(\partial_z\psi^{(1)}_\rho)^2  - \iint_{\mathcal{R}(s_0)} \mathcal{A}_2 \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi^{(1)}_\rho  \psi^{(1)}_\rho  - \iint_{\mathcal{R}(s_0)} \partial_z(w \br{r}^2V_k) \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi^{(1)}_\rho \psi_\rho  \nonumber\\[2\jot]
        &+ \iint_{\mathcal{R}(s_0)} e^{(q_k-\rho)s} \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi^{(1)}_\rho \partial_z (w \br{r}^2 \mathcal{E}_{p,0}) .\label{eq:prop33:temp1.0}
    \end{align}
    We turn to estimating the various bulk terms, starting with the term proportional to $\mathcal{A}_2$. Since $\ell \geq 1$ we have $\ell(\ell+1) \geq 2$. Define $\ell^2_r \doteq \ell(\ell+1)-2$. 
    
    Applying (\ref{34:est2})-(\ref{34:est4}) gives the pair of localized estimates  
    \begin{align}
        \sup_{s \geq 0} \| \mr{r}\bigg( \mathcal{A}_2 - \frac{\ell^2_r}{w\br{r}^2}\bigg)\|_{L^\infty_z([-1,-\frac{1}{2}])} &\lesssim k^2, \label{eq:prop33:temp2.0}\\
        \sup_{s \geq 0} \| \mathcal{A}_2 - \frac{\ell^2_r}{w\br{r}^2} \|_{L^2_z([-\frac{1}{2},0])} &\lesssim k^2, \label{eq:prop33:temp3.0}
    \end{align}
    holding uniformly in $s$. Observe that (\ref{eq:prop33:temp2.0}) captures a cancellation in top order powers of $\mr{r}$ near the axis. Therefore
    \begin{align}
        \iint_{\mathcal{R}(s_0)} &\mathcal{A}_2 \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi^{(1)}_\rho  \psi^{(1)}_\rho \nonumber  \\[\jot]
        &=  \frac{1}{2}\iint_{\mathcal{R}(s_0)} \frac{\ell^2_r}{w \br{r}^2} \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \big(\psi_\rho^{(1)}\big)^2 + \iint_{\mathcal{R}(s_0)} \bigg(\mathcal{A}_2-\frac{\ell^2_r}{w \br{r}^2} \bigg)\frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi_\rho^{(1)} \psi_\rho^{(1)} \label{eq:prop33:temp4.0}
      \end{align} 
      For $k$ sufficiently small the first term may be integrated by parts to produce favorable bulk terms (cf. (\ref{34:est1}))
      \begin{align*}
          \omega \iint_{\mathcal{R}(s_0)}  \frac{\ell_r^2}{w\br{r}^2}\frac{|z|^{2\omega-1}}{\br{r}^4} \big(\psi_\rho^{(1)}\big)^2 + \frac12 \iint_{\mathcal{R}(s_0)}  \frac{\ell_r^2}{w\br{r}^2} \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \log(w\br{r}^6) \big(\psi_\rho^{(1)}\big)^2.
      \end{align*}
      We have dropped boundary terms at the axis, noting that these terms appear only for $\ell \geq 2$, for which we have $\psi_{\rho}^{(1)} \lesssim \br{r}^4.$ This decay is fast enough to overwhelm the inverse powers of $\br{r}$ appearing the integrand. 
    
      The latter term in (\ref{eq:prop33:temp4.0}) gives, after applying the localized estimates (\ref{eq:prop33:temp2.0})-(\ref{eq:prop33:temp3.0}), the Hardy inequality (\ref{hardy1}), and Lemma \ref{lemma:basic1dintegral}, 
    \begin{align*}
        \Bigg| \iint_{\mathcal{R}(s_0)} &\bigg(\mathcal{A}_2-\frac{\ell^2_r}{w \br{r}^2} \bigg)\frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi_\rho^{(1)} \psi_\rho^{(1)} \Bigg| \\[2\jot]
        &\lesssim k^2 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \leq -\frac{1}{2} \} }} \frac{1}{\br{r}^5} \big|\partial_z \psi_\rho^{(1)} \big| \big| \psi_\rho^{(1)}\big| + \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \geq -\frac{1}{2} \} }} \bigg(\mathcal{A}_2-\frac{\ell^2_r}{w \br{r}^2} \bigg)|z|^{2\omega}\big|\partial_z \psi_\rho^{(1)} \big| \big|\psi_\rho^{(1)}\big| \\[2\jot]
        &\lesssim k^2 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \leq -\frac{1}{2} \} }} \frac{1}{\br{r}^4} \big(\partial_z \psi_\rho^{(1)} \big)^2 + k^2 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \leq -\frac{1}{2} \} }} \frac{1}{\br{r}^6}\big( \psi_\rho^{(1)} \big)^2 \\[2\jot]
        &+ \delta_1^{-1}\iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \geq -\frac{1}{2} \} }} \bigg(\mathcal{A}_2-\frac{\ell^2_r}{w \br{r}^2} \bigg)^2 |z|^{2\omega}\big( \psi_\rho^{(1)} \big)^2 + \delta_1 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \geq -\frac{1}{2} \} }} |z|^{2\omega}\big(\partial_z \psi_\rho^{(1)} \big)^2 \\[2\jot]
        &\lesssim (\delta_1+ k^2) \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} \big(\partial_z \psi_\rho^{(1)} \big)^2 + \delta_1^{-1}\int_{0}^{s_0} \sup_{z \in [-\frac12, 0]} \big| |z|^{\omega}\psi_\rho^{(1)} \big|^2 \bigg( \int_{-\frac12}^{0}\bigg(\mathcal{A}_2-\frac{\ell^2_r}{w \br{r}^2} \bigg)^2 dz\bigg) ds \\[2\jot] 
        &\lesssim (\delta_1+ k^2) \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} \big(\partial_z \psi_\rho^{(1)} \big)^2 + \delta_1^{-1}k^4 \int_0^{s_0}\sup_{z \in [-\frac12, 0]} \big| |z|^{\omega}\psi_\rho^{(1)} \big|^2 ds \\[2\jot]
        &\lesssim (\delta_1+ k^2) \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} \big(\partial_z \psi_\rho^{(1)} \big)^2 + \delta_1^{-1}k^4 \iint_{\mathcal{R}(s_0)} |z|^{2\omega}\big(\partial_z \psi_\rho^{(1)} \big)^2 \\[2\jot]
        &\lesssim (\delta_1+ k^2) \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} \big(\partial_z \psi_\rho^{(1)} \big)^2.
    \end{align*}
    A similar analysis using (\ref{eq:potentialest1}), (\ref{34:est3}) gives for the second bulk term in (\ref{eq:prop33:temp1.0})
    \begin{align*}
    \Bigg|\iint_{\mathcal{R}(s_0)} &\partial_z(w \br{r}^2V_k) \frac{|z|^{2\omega}}{\br{r}^4}\partial_z \psi^{(1)}_\rho \psi_\rho  \Bigg| \nonumber\\
    &\lesssim \delta_1^{-1} \iint_{\mathcal{R}(s_0)} \big(\partial_z(w \br{r}^2V_k)\big)^2\frac{|z|^{2\omega}}{\br{r}^4} (\psi_\rho)^2 + \delta_1\iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} (\partial_z \psi^{(1)}_\rho)^2 \nonumber\\[2\jot]
    &\lesssim \delta_1^{-1}k^4 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \leq -\frac{1}{2} \} }} \frac{1}{\br{r}^2} (\psi_\rho)^2 + \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \geq -\frac{1}{2} \} }}(\partial_z(w V_k))^2 |z|^{2\omega} (\psi_\rho)^2  + \delta_1 \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} (\partial_z \psi^{(1)}_\rho)^2  \\
    &\lesssim \delta_1^{-1}k^4 \iint\limits_{\substack{\mathcal{R}(s_0) \\ \{z \leq -\frac{1}{2} \} }} \frac{1}{\br{r}^4} (\psi_\rho^{(1)})^2 + k^4 \int_{0}^{s_0} \sup_{z \in [-1,0]} \big||z|^\omega  \psi_\rho \big|^2 + \delta_1 \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} (\partial_z \psi^{(1)}_\rho)^2  \\
    &\lesssim (\delta_1^{-1}+1) k^4 \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} ( \psi^{(1)}_\rho)^2 + \delta_1 \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} (\partial_z \psi^{(1)}_\rho)^2 \\
    &\lesssim \delta_1 \iint_{\mathcal{R}(s_0)} \frac{|z|^{2\omega}}{\br{r}^4} (\partial_z \psi^{(1)}_\rho)^2.
    \end{align*}
    
    The remaining bulk term in (\ref{eq:prop33:temp1.0}) depends on $\mathcal{E}_{p,0}$. The calculation proceeds by the strategy above, in order to handle the $\br{r}$ weights near the axis. The term here is not-borderline in terms of $\br{r}$ weights, has all terms proportional to $k^2$, and has no $\ell$-dependence. Therefore one may simply take $k$ small to absorb this term, at the cost of a small loss in the $\partial_z \psi_\rho^{(1)}$ bulk term.
    
    Collecting terms, we arrive at the stated estimate.

==> safekeeping.tex <==
\section{Proof concluded}
\label{sec:proof}
In order to prove Theorem \ref{theorem:mainthm}, we require two additional preliminaries. The first, discussed in Section \ref{subsec:proofcompleted_1}, is a physical space scattering result relating \textit{regularity} for null data to \textit{decay} for spacelike data. We also require a sharp decay result for inhomogeneous wave equations with spacelike data, in a region $\{x \leq x_0\}$ close to the axis. This is proved in Section \ref{subsec:proofcompleted_2}, relying on the spectral theory constructions of Section \ref{sec:scattering}. Finally, in Section \ref{subsec:proofcompleted_3} we integrate these threads with muliplier estimates to prove the theorem.

Theorem \ref{theorem:angularthm} is proved entirely using the multiplier estimates established in Section \ref{sec:multipliers}, and is logically independent of the other results in this section. 

\subsection{Backwards scattering}
\label{subsec:proofcompleted_1}
The main result of this section establishes a correspondence between null data $(r\varphi)_0(v) \in \mathcal{C}^{\alpha}_{(hor)}([-1,0])$ on $\{u=-1\}$ and spacelike data $((r\varphi)_0(x), \partial_t (r\varphi)_0(x))$ on $\{t=0\}$. We will assume throughout that all data is spherically symmetric, and thus $\ell$-dependent terms in the wave equation.

\begin{prop}
    \label{prop:backwardsdecay}   
    Fix $\alpha \in (1,2)$, and outgoing null initial data $h_0(v) = (r\varphi)_0(v) \in C^{\alpha}_{(hor)}([-1,0])$. Let $\psi(u,v) = (r\varphi)(u,v)$ denote the unique solution to the linear wave equation (\ref{sec2.5:eq2}) in $\{u \geq -1\}$. There exists spacelike data $(f_0(x),f_1(x)) \in \mathcal{D}_\infty^{\alpha, 4}(\mathbb{R}_+) \times \mathcal{D}_\infty^{\alpha, 3}(\mathbb{R}_+)$ for $(r\varphi,\partial_t(r\varphi))$ on $\{t=0\}$ such that the unique solution $\wt{\psi}(t,x)=(r\varphi)(t,x)$ to the linear wave equation (in hyperbolic coordinates) (\ref{eq:wavehyper}) on $\{t \geq 0\}$ satisfies the following:
    \begin{itemize}
        \item $\wt{\psi}(t,x) \in C^{4}_{t,x}(\{t \geq 0\})$
        \item Written in double-null coordinates, $\wt{\psi}(u,v)$ coincides with $\psi(u,v)$ in their common domain of definition.
        \item For any $T > 0$ fixed, the estimate holds 
        \begin{equation}
            \label{eq:propbackscat_1}
            \sup_{t\in[0,T]}\sum_{j=0}^4\|\partial_t^j\wt{\psi}(t,\cdot)\|_{\mathcal{D}^{\alpha,4-j}_\infty(\mathbb{R}_+)} \lesssim_T \|h_0 \|_{\mathcal{C}^{\alpha}_{(hor)}([-1,0])}.
        \end{equation}
    \end{itemize}
    If we moreover assume $h_0(z) \in C^{\alpha,\delta}_{(hor)}([-1,0])$ for some $\delta \in (0,1)$, then there exists a $c_0 \in \mathbb{R}$ such that the induced data $(f_0(x),f_1(x))$ lies in $\wt{\mathcal{D}}^{\alpha, 4, \delta,c_0}_\infty(\mathbb{R}_+) \times  \wt{\mathcal{D}}^{\alpha, 3, \delta,c_0}_\infty(\mathbb{R}_+)$. There exists a $\delta'>0$ such that for all $t \in [0,T]$, $\wt{\psi}(t,x) - c_0 e^{\alpha q_k (t-x)} \in \mathcal{D}^{\alpha+\delta',4}_{\infty}(\mathbb{R}_+),$ and we have the estimate 
    \begin{equation}
        \label{eq:propbackscat_1.5}
       |c_0| +  \sup_{t\in[0,T]} \sum_{j=0}^4 \|\partial_t^j\big(\wt{\psi}(t,\cdot) - c_0 e^{\alpha q_k (t-x)}\big)\|_{\mathcal{D}^{\alpha+\delta',4-j}_\infty(\mathbb{R}_+)} \lesssim_T \|h_0 \|_{\mathcal{C}^{\alpha,\delta}_{(hor)}([-1,0])}.
    \end{equation}
    \end{prop}

\begin{proof}

\vspace{.5em}
\noindent
\textbf{Posing compatible ingoing data:} 
We construct spacelike data $(f_0(x),f_1(x))$ by solving the backwards characteristic problem for (\ref{sec2.5:eq2}) with data along $\{u=-1\} \cup \{v=0, u \leq -1\}$. To render this problem well-posed, we specify appropriate data for $r\varphi$ along the ingoing null component, denoted $h_1(u)$. We claim this ingoing data can be chosen such that the following conditions hold:
\begin{enumerate}
    \item $\text{supp} \ h_1(u) \in [-2,-1]$, and $h_1 \in C^4_{u}([-2,-1])$, with $\|h_1 \|_{C^4_u([-2,-1])} \lesssim \|h_0 \|_{C^\alpha_{(hor)}([-1,0])}$
    \item $h_1(-1) = h_0(0)$
    \item $\partial_u^{j} h_1(-1) = \partial_u^j \psi(-1,0), \quad 0 \leq j \leq 4$
    \item $\text{supp} \ \partial_v \wt{\psi}(u,0) \in [-2,-1]$
    \item  $\big||v|^{j- \alpha} \partial_v^j \wt{\psi}(u,0)\big| \lesssim 1, \quad 2 \leq j \leq 4$
\end{enumerate}
To briefly comment on the significance of these conditions, we note that (1)--(2) are natural requirements of compatibility with outgoing data and compact support. Condition (4) requires not only $r\varphi(u,0)$ to be compactly supported in $u$, but additionally\footnote{Note this is not possible for every wave equation of the form (\ref{sec2.5:eq2}). In Minkowski space, the wave equation reduces to a conservation law $\partial_u \big(\partial_v (r\varphi)\big) = 0$, implying the derivative can only be compactly supported if additional conditions are imposed on $h_0(v)$.} $\partial_v(r\varphi)(u,0)$. Condition (3) is forced by the requirement of $C^4$ gluing of $\psi$ and $\wt{\psi}$ across $\{u=-1\}$. This is forced by the presence of an axis. Finally, condition (5) asserts that the singular bounds on $h_0(u)$ are propagated to the past.

Continuing with the proof, it is direct that we can choose $h_1(u)$ to satisfy conditions (1)--(3), which only constrain the jet of $h_1$ at the point $u=-1$. The quantitative estimate in (1) moreover follows from the local well-posedness estimates for $\psi$, i.e. (\ref{eq:localexist_bound}). 

To see condition (4), we restrict (\ref{sec2.5:eq2}) to $\{v=0\}$ and integrate in $u$. 
\begin{equation}
    \label{eq:backscatproof:temp1}
    \partial_v \wt{\psi}(u,0) = h_0'(0) + \int_{u}^{-1} \bigg(\frac{\lambda(-\nu)\mu}{(1-\mu)r^2}\bigg)(u',0) h_1(u')du',
\end{equation}
By assumption on $(\epsilon_0,k)$-admissible spacetimes, we can expand
\begin{equation*}
    \bigg(\frac{\lambda(-\nu)\mu}{(1-\mu)r^2}\bigg)(u,0) = \frac{c_k + \epsilon_0 k^2 g(u)}{|u|^{2-k^2}}
\end{equation*}
for a non-zero constant $c_k$ and function $g(u)$ supported in $[-2,-1]$. It now suffices to choose $h_1$ such that (\ref{eq:backscatproof:temp1}) evaluates to zero when $u=-2$. 

Finally, condition (5) will follow from the set of conservation laws
\begin{align*}
    \partial_u (|v|^{j-\alpha}\partial_v^j \wt{\psi})(u,0) = 0, \quad 2\leq j \leq 4.
\end{align*}
These follow inductively in $j$ by commuting (\ref{sec2.5:eq2}) with $|v|^{j-\alpha}\partial_v^{j-1}$, and applying the regularity (\ref{eq:potentialest3.5}).

\vspace{1em}
\noindent
\textbf{Pointwise bounds:}
We turn to estimating the solution in a characteristic rectangle $\mathcal{B} = \{u \leq -1, v \geq -\frac12 \}.$ In the following, let $C(h_1,h_2)$ denote any constant depending on the $C^{\alpha}_{(hor)}([-1,0])$ norm of $h_1$, and the $C^4_u([-2,-1])$ norm of $h_2$. We first show the bound
\begin{equation}
    \label{eq:backscatproof:temp2}
    \|\wt{\psi}\|_{C^1_{u,v}(\mathcal{B})} + \||u| \partial_u \wt{\psi}\|_{L^\infty_{u,v}(\mathcal{B})} \leq C(h_1,h_2),
\end{equation} 
which will follow from a multiplier estimate. We choose to work in similarity coordinates for convenience, and estimate (\ref{eq:wavesimfull}). Multiplying by $\partial_s \wt{\psi}$ and integrating by parts in $\mathcal{R}(s_0,0)$ for an arbitrary $s_0 < 0$ yields 
\begin{align*}
    \frac{1}{2}\int_{s_0}^{0}&(\partial_s \wt{\psi})^2(s,0)ds  + \frac{1}{2}q_k \int_{\{s=0\}} |z| (\partial_z \wt{\psi})^2(0,z)dz +  \frac{1}{2}\int_{\{s=0\}}V(0,z)  \wt{\psi}^2(0,z) dz \\[\jot]
    &+ \frac{1}{2}\iint_{\mathcal{R}(s_0,0)}\partial_s(V-V_k) \wt{\psi}^2(s,z) dsdz = \frac{1}{2}q_k \int_{\{s=s_0\}} |z| (\partial_z \wt{\psi})^2(s_0,z)dz+  \frac{1}{2}\int_{\{s=s_0\}}V(s_0,z)  \wt{\psi}^2(s_0,z) dz.
\end{align*}
We have used that $\partial_s V_k = 0$ to drop the corresponding bulk term. By the assumptions on $(\epsilon_0,k)$-admissible spacetimes, the remaining bulk term is supported in $\{u \in [-2,-1]\}$ and satisfies a pointwise bound in terms of $\epsilon_0$. Choosing this parameter sufficiently small, taking the supremum over $s \in [s_0,0]$, and absorbing the bulk term, we conclude that the multiplier estimate controls $\|\wt{\psi} \|_{L^2_z(\{s=s_0\})}$. In double-null coordinates we have
\begin{equation}
    \label{eq:backscatproof:temp3}
    \sup_{u' \leq -1}\|\wt{\psi} \|_{L^2_v(\{u=u'\})} \leq C(h_0,h_1)|u|^{\frac12 q_k}.    
\end{equation}
This bound, in combination with integration along characteristics, will give (\ref{eq:backscatproof:temp2}). We sketch the argument here.

Denoting the zeroth order coefficient in (\ref{sec2.5:eq2}) by $P(u,v),$ we can estimate $|P(u,v)| \lesssim |u|^{-2+k^2}.$ In particular, this term rapidly decays as $|u| \rightarrow \infty$. We now integrate (\ref{sec2.5:eq2}) as an equation for $\partial_u \wt{\psi}$ and estimate $P(u,v)\wt{\psi}$ via Cauchy-Schwarz. It follows that $\partial_u \wt{\psi}$ decays at an integrable rate, and thus $\wt{\psi}$ and $\partial_u \wt{\psi}$ are bounded. Integrating (\ref{sec2.5:eq2}) again as an equation for $\partial_v \wt{\psi}$ gives boundedness of this quantity as well.

\vspace{.5em}
\noindent
A corollary of (\ref{eq:backscatproof:temp2}) are the higher order bounds 
\begin{equation}
    \label{eq:backscatproof:temp4}
    \||u|^{j}\partial_u^j \wt{\psi}\|_{L^\infty_{u,v}(\mathcal{B})}+\||v|^{j-\alpha}\partial_v^j \wt{\psi}\|_{L^\infty_{u,v}(\mathcal{B})} \leq C(h_1,h_2) \quad 2\leq j \leq4.
\end{equation}
These follow inductively in $j$ by commuting (\ref{sec2.5:eq2}) with $\partial_u^j, \ |v|^{j-\alpha} \partial_v^{j-1}$, applying (\ref{eq:backscatproof:temp2}), and integrating in the $v$, $u$ directions respectively. The initial data terms along $\{u=-1\}$ limit the regularity of $\partial_v^j \wt{\psi}$ in (\ref{eq:backscatproof:temp4}).

The sharp bounds (\ref{eq:propbackscat_1}) now follow. Integrating the ${j=2}$ estimate in (\ref{eq:backscatproof:temp4}) in $v$ implies that for all ${u \leq -2}$, 
\begin{equation}
    \label{eq:backscatproof:temp5}
    |\partial_v \wt{\psi}(u,v)| \leq C(h_0,h_1)|v|^{\alpha-1},
\end{equation}
and after integrating again,
\begin{equation}
    \label{eq:backscatproof:temp6}
    |\wt{\psi}(u,v)| \leq C(h_0,h_1)|v|^{\alpha},
\end{equation}

It now suffices to collect (\ref{eq:backscatproof:temp2}), (\ref{eq:backscatproof:temp4}), (\ref{eq:backscatproof:temp5}), (\ref{eq:backscatproof:temp6}), and apply the coordinate transformations between double-null and hyperbolic coordinates,
\begin{align*}
    \partial_t = |u|\partial_u + q_k |v| \partial_v, \ \ \partial_x =  -|u|\partial_u + q_k |v| \partial_v,
\end{align*}
to conclude (\ref{eq:propbackscat_1}).

\vspace{1em}
\noindent
\textbf{Refinement for data in $\mathcal{C}^{\alpha,\delta}_{(hor)}$:}
Finally we examine the case of initial data $h_0(u) \in \mathcal{C}^{\alpha,\delta}_{(hor)}([-1,0])$, and show the sharper (\ref{eq:propbackscat_1.5}). By Lemma \ref{lem:holderspacedecomp} and linearity, it is sufficient to consider $h_0(u) = c_0|u|^{\alpha}$ for a constant $c_0$. Define $c_j \doteq |u|^{j-\alpha}\frac{d^j}{du^j}h_0(u),$ $j \geq 0$. 

By the same argument that leads to (\ref{eq:backscatproof:temp4}), we may commute (\ref{sec2.5:eq2}) inductively by $|v|^{j-\alpha}\partial_v^{j-1}$ and estimate, giving
\begin{align*}
    \partial_u \big(|v|^{j-\alpha}\partial_v^j \wt{\psi}\big) = O_{L^\infty_{u,v}}(|v|^{2-\alpha}|u|^{-2+k^2}) \quad 2\leq j \leq 4.
\end{align*}
Integrating in $u$ from data, we see that the contribution from the initial data term dominates the expansion for $\partial_v^j \wt{\psi}$:
\begin{equation}
    \label{eq:backscatproof:temp7}
    |v|^{j-\alpha}\partial_v^j \wt{\psi}(u,v) = c_j + O_{L^\infty_{u,v}}(|v|^{2-\alpha}) \quad 2\leq j \leq 4.
\end{equation}
Integrating the $j=2$ expansion further yields 
\begin{align}
    \partial_v \wt{\psi}(u,v) &= \partial_v \wt{\psi}(u,0) + c_1 |v|^{\alpha-1} + O_{L^\infty_{u,v}}(|v|) \label{eq:backscatproof:temp8}\\
    \wt{\psi}(u,v) &= h_1(u) + c_0  |v|^{\alpha} + O_{L^\infty_{u,v}}(|v|^2). \label{eq:backscatproof:temp9}
\end{align}
If we now define $\wt{\psi}_{reg}  \doteq \wt{\psi} - c_0 |v|^{\alpha}$, it follows from the estimates on $u$-derivatives (\ref{eq:backscatproof:temp2})--(\ref{eq:backscatproof:temp4}), as well as the expansions (\ref{eq:backscatproof:temp7})--(\ref{eq:backscatproof:temp9}), that we have for some $\delta' > 0$
\begin{equation}
   \sup_{t' \in [0,T]} \| e^{(\alpha+\delta')x}\wt{\psi}_{reg} \|_{C^4_{t,x}(\{t=t'\})} \lesssim_T \|h_0\|_{C^{\alpha,\delta}_{(hor)}([-1,0])}.
\end{equation}
\end{proof}



\subsection{Leading order expansion in the near-axis region}
\label{subsec:proofcompleted_2}
In this section we establish a leading order expansion for the solution to the following inhomogeneous problem:
\begin{equation}
    \label{eq:forcedeqn1}
    \begin{cases}
    &\partial_t^2 \psi - \partial_x^2 \psi  + 4q_k e^{-2q_k x}V_k(x) \psi =  f(t,x), \\[\jot]
        &\psi(t,0) =0,  \\[\jot]
        &(\psi(0,x), \partial_t \psi(0,x)) = (0,0),
    \end{cases}
\end{equation}
where the inhomogeneity satisfies 
\begin{equation}
    \label{52:forcingassTOTAL}
    \begin{cases}
    &f(t,x) \in C^3_{t,x}(\mathbb{R}_+ \times \mathbb{R}_+),   \\[\jot]
    &\text{supp}\ f(\cdot,x) \in [1,\infty) \ \text{for all} \ x,   \\[\jot]
    &\sup_{\{t \geq 0\}} \sum_{j=0}^3 e^{2t}\|\partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} \leq C, 
    \end{cases}
\end{equation}
for constants $\beta \in (1,2)$ and $C > 0$. The analysis will depend on the spatial decay of $f(t,x)$, manifest in the constant $\beta$. In the range $\beta > p_k$, corresponding (by Proposition \ref{prop:backwardsdecay}) to null data \textit{strictly more regular} than that of the background solution, we show that the solution to (\ref{eq:forcedeqn1}) converges in compact sets to a constant multiple of the $k$-self-similar radius function $r_k$. 

Convergence to constants will not in general hold for the \textit{threshold regularity} case ${\beta = p_k}$, or the \textit{sub-threshold regularity} case ${\beta < p_k}$. For these latter cases, we impose an additional assumption, denoted $(A_\beta)$.
\begin{enumerate}
    \item[$(A_{\beta})$] There exists a decomposition $f(t,x) = c_0 \chi_b(t) e^{\beta q_k(t-x)} + f_2(t,x)$, with $c_0$ a constant, $\chi_b(t)$ a smooth, non-negative bump function with support in $[1,2]$, and $f_2(t,x)$ a function satisfying the assumptions (\ref{52:forcingassTOTAL}) for some $\beta' = \beta+\delta$.
\end{enumerate}

For initial data with $\beta = p_k$, which moreover satisfies $(A_{p_k})$, we establish exponential convergence in compact sets to a linear combination of terms of the form $r_k, g(x)r_k,  r_k t$, where $g(x)$ is a locally bounded function. The first two terms correspond to a bounded scalar field; the final term, however, is novel to the threshold regularity case, and corresponds to a scalar field growing like $-\log |u|$. Note this is precisely the behavior of the background $k$-self-similar scalar field $\phi_k(u,v)$.

Finally, in the case $\beta <p_k$, the solution converges exponentially in compact sets to a term which grows as $e^{-\beta q_k t}$; in particular, the solution can grow with a rate strictly between the self-similar and blue-shift rate.

\begin{prop}
    \label{prop:resonanceexp}
    Fix an $(\epsilon_0,k)$-admissible background, with $k$ sufficiently small. Choose parameters $\beta \in (1,2)$, $x_0>0$, and let $\eta \in (0,\frac12)$ be the parameter defined in Section \ref{sec:scattering} (cf. Remark \ref{rmk:etafixed}). Let $\psi(t,x)$ denote a solution to (\ref{eq:forcedeqn1})--(\ref{52:forcingassTOTAL}). We distinguish various cases below:

    \vspace{.5em}
    \noindent
    \underline{$\beta > p_k$: } Define $\beta_* = \min(\beta q_k, 1+\eta),$ and fix any $\beta_*' < \beta_*$. Then there exists a constant $c^{(0)}_{\infty}$ independent of $x_0$, and a constant $C_{x_0, \beta_*'} \lesssim (1+x_0) e^{\beta_*' x_0},$ such that
    \begin{equation}
        \label{eq:resonanceexp}
        \sup_{\{t \geq 0\}} \sum_{j=0}^2 \|e^{\beta_*' t}\partial_t^j(\psi - c^{(0)}_{\infty} r_k) \|_{C^{2-j}_x([0,x_0])} \lesssim C_{x_0, \beta_*'} \sup_{\{t \geq 0\}} \sum_{j=0}^3 e^{2t}\|\partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)}.
    \end{equation}
    Moreover, $|c^{(0)}_\infty|$ can be estimated by the right hand side of (\ref{eq:resonanceexp}).

    \vspace{.5em}
    \noindent
    \underline{$\beta = p_k$, $(A_{p_k})$: } Assume $f(t,x)$ satisfies $(A_{p_k})$ with constants $c_0, \delta$. For any $\delta' < \delta$, there exists an $L^\infty_{loc}(\mathbb{R}_+)$ function $g^{(1)}_\infty(x)$ and constant $c_\infty^{(1)}$ independent of $x_0$, and a constant $C_{x_0, \delta'} \lesssim (1+x_0)e^{(1+\delta')x_0}$, such that 
    \begin{align}
        \sup_{\{t \geq 0\}} \sum_{j=0}^2 \| e^{(1+\delta')t}\partial_t^j \big(\psi -  c_\infty^{(1)}  r_k  t &-  g^{(1)}_\infty(x)r_k\big)\|_{C^{2-j}_x([0,x_0])} \nonumber \\[\jot]
        &\leq C_{x_0, \delta'} \bigg(|c_0| + \sup_{\{t \geq 0\}} \sum_{j=0}^3 e^{2t}\| \partial_t^j f_2 \|_{\mathcal{D}^{p_k+\delta,0}_\infty(\mathbb{R}_+)} \bigg). \label{eq:resonanceexp1}
    \end{align}
    Moreover, $|c^{(1)}_\infty|$, $\|g_{\infty}^{(1)}\|_{L^\infty_x([0,x_0])}$ can be estimated by the right hand side of (\ref{eq:resonanceexp1}).

    \vspace{.5em}
    \noindent
    \underline{$\beta < p_k$, $(A_{\beta})$: } Assume $f(t,x)$ satisfies $(A_{\beta})$ with constants $c_0, \delta$. For any $\delta' < \delta$, there exists a $L^\infty_{loc}(\mathbb{R}_+)$ function $g_\infty^{(2)}(x)$ and a constant $C_{x_0,\delta'} \lesssim (1+x_0)e^{(\beta+\delta')x_0}$ such that 
    \begin{align}
        \sup_{t}\sum_{j=0}^2 \|e^{(\beta+\delta')t} \partial_t^j (\psi - &g_\infty^{(2)}(x)e^{-\beta q_k t}) \|_{C^{2-j}_x([0,x_0])} \nonumber\\[\jot]
        &\leq  C_{x_0,\delta'}\bigg(|c_0| +  \sup_{\{t \geq 0\}} \sum_{j=0}^3 e^{2t} \|\partial_t^j f_2 \|_{\mathcal{D}^{\beta+\delta,0}_\infty(\mathbb{R}_+)} \bigg). \label{eq:resonanceexp1.1}
    \end{align}
    Moreover, $\|g_{\infty}^{(2)}\|_{L^\infty_x([0,x_0])}$ can be estimated by the right hand side of (\ref{eq:resonanceexp1.1}). Finally, if $c_0 \neq 0$, then the function $g_\infty^{(2)}(x)$ does not identically vanish.
    \end{prop}


\begin{proof}
By a density argument, it suffices to establish (\ref{eq:resonanceexp})--(\ref{eq:resonanceexp1.1}) for $f(t,x) \in C^\infty_{t,x}$. Given that $f(t,x)$ is supported in $\{t \geq 1\}$, we may then extend $\psi(t,x)$ to $\mathbb{R}\times \mathbb{R}_+$ by $\psi(t,x) = 0$ for $t \leq 0$, and $\psi(t,x) \in C^\infty_{t,x}$.

For $\sigma \in \mathbb{C}$, let $\wh{\psi}(\sigma,x)$ denote the Fourier-Laplace transform of $\psi$ in the $t$ variable, where we use the sign convention
\begin{equation}
    \wh{\psi}(\sigma,x) = \int_{\mathbb{R}}e^{i \sigma t} \psi(t,x) dt.
\end{equation}
We have established boundedness in $t$ for $\psi(t,x)$ in Lemma \ref{lem:pointwiseboundforeasywaveequation}, and thus this transform is well-defined for all $\Im \sigma > 0$. For fixed $\sigma$ in the upper half plane we have the regularity $\wh{\psi}(\sigma,x) \in C^\infty_x(\mathbb{R}_+)$, as well as the bound $\sup_{x}|(1+\sqrt{x})^{-1}\wh{\psi}(\sigma,x)| < \infty$. By (\ref{52:forcingassTOTAL}) the transform $\hat{f}(\sigma,x)$ is well-defined for $\{\Im \sigma > -2\}$, and $\sup_{x}|e^{\beta q_k x}\hat{f}(\sigma,x)| < \infty$ holds. In the following, we write $\wh{\psi}_{\sigma}(x) \doteq \wh{\psi}(\sigma,x)$, and similarly $\wh{f}_{\sigma}(x) \doteq \wh{f}(\sigma,x)$.

It follows that $\wh{\psi}_{\sigma}(x)$ solves 
\begin{align*}
    \begin{cases}
    -\frac{d^2}{dx^2}\wh{\psi}_{\sigma}(x) + (4q_k e^{-2q_k x}V_k(x) -\sigma^2)\wh{\psi}_{\sigma}(x) = \wh{f}_\sigma(x) \\[\jot]
    \wh{\psi}_{\sigma}(0)=0,
    \end{cases}
\end{align*}
with at most polynomial growth at infinity. By Lemma \ref{lem:resolventuniquness} we must have
\begin{equation*}
    \wh{\psi}_{\sigma}(x) = (R(\sigma) \wh{f}_\sigma)(x).
\end{equation*}
The Fourier-Laplace inversion formula now provides the following representation formula for $\psi$, cutoff to a range $x \leq x_0$: 
\begin{align}
    \label{eq:resonanceexp1.5}
    \rho_{x_0}(x)\psi(t,x) = \frac{1}{2\pi}\int_{\{\Im \sigma = \eta \}} e^{-i\sigma t}(\rho_{x_0}R(\sigma)\wh{f}_\sigma)(x) d\sigma.
\end{align}
The integration takes place on a horizontal contour in the upper half plane.
As $f(t,x)$ is smooth in the $t$ coordinate, $\wh{f}_\sigma(x)$ is rapidly decaying in $\sigma$ for $|\Re \sigma| \gg 1$. Therefore, the integral converges pointwise in $x$. 

We now specialize to the case $\beta > p_k$. Arguments for the remaining cases follow similarly, and are sketched at the end of the proof. In the high regularity setting with $\beta > p_k$ (and therefore $\beta_* > 1$), the integrand in (\ref{eq:resonanceexp1.5}) is defined and meromorphic in $\sigma$ for $\sigma \in \mathbb{I}_{(-\beta_*,\eta]}$. Choosing $\epsilon_*$ small such that $-\beta_* + \epsilon_* < -1$, the goal is to deform the contour of integration in (\ref{eq:resonanceexp1.5}) to $\{\Im \sigma = -\beta_* + \epsilon_*\}$, picking up a contribution from the unique pole at ${\sigma = -i}$.

Fix a small constant $\epsilon_1$ and a large constant $R > 0$, and define the oriented contours
\begin{align}
    \label{eq:resonanceexp_prooftemp0}
    \begin{cases}
    \gamma_{\epsilon_1} &= -i +  \epsilon_1 e^{-i \theta} \hspace{3.3em} \theta \in [0,2\pi) \\
    \Gamma^{\pm}_{1,R} &= \eta i  \pm R \pm t \hspace{4em} t \in [0,\infty) \\
    \Gamma^{\pm}_{2,R} &= \eta i \pm R - i t \hspace{3.65em} t \in [0, \eta + \beta_* - \epsilon_1] \\ 
    \Gamma_{3,R} &= (-\beta_* + \epsilon_*)i + t \hspace{1.85em}   t \in [-R,R]
    \end{cases}
\end{align}
as well as the path $P_R \subset \mathbb{C}$
\begin{align*}
    P_R \doteq -\Gamma^{-}_{1,R} \cup -\Gamma^{-}_{2,R} \cup \Gamma_{3,R} \cup \Gamma^{+}_{2,R} \cup \Gamma^{+}_{1,R}.
\end{align*}
We may deform the contour in (\ref{eq:resonanceexp1.5}) in a compact subset of $\mathbb{C}$, giving 
\begin{align}
    \label{eq:resonanceexp_prooftemp.5}
    \rho_{x_0}(x)\psi(t,x) &= \frac{1}{2\pi}\int_{\gamma_{\epsilon_1}}e^{-i\sigma t}(\rho_{x_0}R(\sigma)\wh{f}_\sigma)(x) d\sigma + \frac{1}{2\pi}\int_{P_R}e^{-i\sigma t}(\rho_{x_0}R(\sigma)\wh{f}_\sigma)(x) d\sigma.
\end{align}
Appealing to the analysis (\ref{eq:residueatpole})--(\ref{eq:residueatpole1}) of $R(\sigma)$ near ${\sigma=-i}$, the integral over the closed loop $\gamma_{\epsilon_1}$ is explicitly computable as  
\begin{equation}
    \label{eq:resonanceexp_prooftemp1}
    -i c_* \rho_{x_0}(x)e^{x}e^{-t}\mr{r}(x)\int_0^\infty e^{x'}\mr{r}(x') \wh{f}_{-i}(x') dx' \doteq c^{(0)}_{\infty} e^{x-t}\rho_{x_0}(x) \mr{r}(x),
\end{equation}
where we have defined the constant $c_{\infty}^{(0)}$ appearing in (\ref{eq:resonanceexp}). Moreover, we can recognize $e^{x-t}\mr{r}(x)$ as $r_k(t,x)$. The integral over $P_R$ will contribute a faster decaying error, which we now estimate. The resolvent estimates (\ref{eq:c0toc2bounds}) are instrumental in bounding derivatives of the resolvent; however, each derivative loses a power of $\sigma$, obstructing convergence of the integrals for $|\Re \sigma| \gg 1$. In this region we regain favorable powers of $|\sigma|$ by exploiting the $t$ regularity of $f(t,x)$. The relevant statement is given in Lemma \ref{lem:associatedlemma_resonanceexp}, proved below. For $0 \leq m + j \leq 2$ apply (\ref{eq:c0toc2bounds}) and (\ref{eq:resonanceexp2}) to give
\begin{align*}
    \sup_{x \in [0,x_0]}\Big| \frac{1}{2\pi} \partial_t^m \partial_x^j \bigg( \int_{ P_R \setminus \Gamma_{3,R}}e^{-i\sigma t}(\rho_{x_0}R(\sigma)\wh{f}_\sigma)(x) d\sigma  \bigg) \Big| &\lesssim_{x_0}  \int_{ P_R \setminus \Gamma_{3,R}}  (1+|\sigma|) \|\hat{f}_\sigma\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} d\sigma  \\[\jot]
     &\lesssim_{x_0}  \sup_{\{t \geq 0\}}\sum_{j=0}^3e^{2t} \| \partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} \int_{ P_R \setminus \Gamma_{3,R}} (1+|\sigma|)^{-2}  d\sigma \\[\jot]
    &\lesssim_{x_0} R^{-1} \sup_{\{t \geq 0\}}\sum_{j=0}^3e^{2t} \| \partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} .
\end{align*}
For fixed $x \leq x_0$, the $C^2_{t,x}$ norm of these boundary integrals with $|\Re \sigma| \geq R$ vanishes as $R \rightarrow \infty$. It remains to estimate the term along $\Gamma_{3,R}$. For this term we also track the dependence on the cutoff $x_0$. For $0 \leq m + j \leq 2$ compute 
\begin{align*}
    \sup_{x \in [0,x_0]}\Big| \frac{1}{2\pi} \partial_t^m \partial_x^j \bigg(\int_{\Gamma_{3,R}} e^{-i\sigma t}(\rho_{x_0}R(\sigma)\wh{f}_\sigma)(x) d\sigma \bigg) \Big|
    &\lesssim (1+x_0)e^{(\beta_*-\epsilon)x_0} e^{-(\beta_*-\epsilon)t} \int_{\Gamma_{3,R}} (1+|\sigma|) \|\hat{f}_\sigma\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} d\sigma  \\[\jot]
    &\lesssim (1+x_0)e^{(\beta_*-\epsilon)x_0} e^{-(\beta_*-\epsilon)t}  \sum_{j=0}^3e^{2t} \| \partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)}.
\end{align*} 
This completes the proof of (\ref{eq:resonanceexp}). To complete the case $\beta > p_k$, we observe that an estimate for $c_{\infty}^{(0)}$ follows from the integral expression (\ref{eq:resonanceexp_prooftemp1}), and a pointwise estimate for $\hat{f}_{-i}(x)$ given by (\ref{eq:resonanceexp2}).

We next consider the cases $\beta = p_k$ and $\beta < p_k$. Note that $\beta_* = \beta q_k \leq 1$. Under the assumption $(A)_{\beta}$, the inhomogeneity $f(t,x)$ decomposes as $f(t,x) = c_0 \chi_b(t)e^{\beta q_k (t-x)} + f_2(t,x)$, for an error $f_2(t,x)$ with strictly better spatial decay. By linearity we may separately estimate the solution to (\ref{eq:forcedeqn1}) with right hand side $f_2(t,x)$. The required estimates (\ref{eq:resonanceexp1}), (\ref{eq:resonanceexp1.1}) follow by analogous techniques as above, precisely because $f_2(t,x)$ has more than enough decay to deform the contour to $\{\Im \sigma = -\beta q_k + \delta'\}$, for some $\delta'$ small enough. 

Assume that $f(t,x) = c_0 \chi_b(t)e^{\beta q_k (t-x)}$, and compute $\hat{f}_\sigma(x) = c_0 \hat{F}(\sigma) e^{-\beta q_k x}$ for an appropriate holomorphic function $\hat{F}(\sigma)$. Let the contours be as in (\ref{eq:resonanceexp_prooftemp0}), with the modification that $\Gamma^{\pm}_{2,R}, \Gamma_{3,R}$ extend only to $\{\Im \sigma = -\beta q_k + \delta' \}$. Equation (\ref{eq:resonanceexp_prooftemp.5}) continues to hold, and the integral over $P_R$ is estimated to give $t$ decay of $e^{-(\beta q_k+\delta')t},$ as expected. 

The remaining contribution arises from the poles of $\rho_{x_0}R(\sigma)e^{-\beta q_k x}$ in $\{\Im \sigma \geq -\beta q_k - \delta'\}$, which were studied in Proposition \ref{lem:extR_sigma_2}. There is either a double pole at $\sigma = -i$ (in the case $\beta = p_k$), or a simple pole at $\sigma = -\beta q_k i$ (in the case $\beta < p_k$). The appropriate resolvent expansions are given by (\ref{eq:resolvexp_extension}), (\ref{eq:resolvexp_extension_2}) respectively. Applying the residue theorem concludes the proof. 
\end{proof}

\begin{lemma}
    \label{lem:associatedlemma_resonanceexp}
    Assume $f(t,x)$ satisfies the conditions (\ref{52:forcingassTOTAL}). Then we have
        \begin{equation} 
            \label{eq:resonanceexp2}
            \sup_{\sigma \in \mathbb{I}_{(-\beta_*,\eta]}}(1+|\sigma|)^3\|\wh{f}_\sigma(x)\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)} \lesssim \sup_{\{t \geq 0\}} \sum_{j=0}^{3}e^{2 t}\|\partial_t^j f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)}.
        \end{equation}
    \end{lemma}
    \begin{proof}
      For $\sigma \in \mathbb{I}_{(-\beta_*,\eta]}, \ 0 \leq m \leq 3$,  estimate 
    \begin{align*}
        |\sigma|^m  |e^{\beta q_k x}\wh{f}_{\sigma}(x)| &=  |\sigma|^m \bigg| \int_{\mathbb{R}} e^{i\sigma t}e^{\beta q_k x} f(t,x)dt\bigg| \\[\jot] 
        &= |\sigma|^m \bigg| \int_{0}^\infty (i \sigma)^{-m}\partial_t^m e^{i\sigma t} e^{\beta q_k x} f(t,x)dt\bigg|\\[\jot]
        &=  \bigg|  \int_{0}^\infty  e^{i\sigma t} e^{\beta q_k x} \partial_t^m  f(t,x)dt\bigg| \\[\jot] 
        &\lesssim \sup_{\{t \geq 0\}}e^{2t} \|\partial_t^m f\|_{\mathcal{D}^{\beta,0}_\infty(\mathbb{R}_+)}.
    \end{align*}
    We have used (\ref{52:forcingassTOTAL}) to drop boundary terms arising from integration by parts in $t$. (\ref{eq:resonanceexp2}) now follows.
    \end{proof}

\subsection{Proof of Theorem \ref{theorem:mainthm}}
\label{subsec:proofcompleted_3}

\subsubsection*{Theorem \ref{theorem:mainthm}(a)}

The proof will essentially be an amalgamation of the techniques developed thus far. To clarify the conceptual structure, we split the argument into various steps.

\vspace{.5em}
\underline{Reduction to spacelike problem}: \
Let $(r\varphi)_0(v) \in C^{\alpha}_{(hor)}([-1,0])$, ${\alpha > p_k}$ denote given spherically symmetric, null initial data along $\{u=-1\}$, and let $\psi(u,v) = (r\varphi)(u,v)$ denote the associated solution to (\ref{sec2.5:eq2}) in $\{u \geq -1\}$. By Proposition \ref{prop:backwardsdecay}, $\psi(u,v)$ may equivalently be described as the solution to (\ref{eq:wavehyper}) for some spacelike initial data $(r\varphi(x), \partial_t(r\varphi)(x)) = (f_0(x),f_1(x)) \in {D}^{\alpha,4}_\infty(\mathbb{R}_+) \times {D}^{\alpha,3}_\infty(\mathbb{R}_+)$ along $\{t=0\}$. The a priori estimate (\ref{eq:propbackscat_1}) holds in any compact (in $t$) region. 

\vspace{.5em}
\underline{Application of leading order resonance expansion}: \
To apply Proposition \ref{prop:resonanceexp}, we need to relate this initial data problem with a forcing problem of the form (\ref{eq:forcedeqn1}). Let $\chi(t) \in C^\infty(\mathbb{R})$ denote an increasing cutoff function, with $\chi(t) = 0$ for $t < 1$, and $\chi(t)=1$ for $t \geq 2$. Define
$$\psi_c \doteq \chi(t) \psi(t,x),$$
as well as the operator 
\begin{equation*}
    \mathcal{T}_k \doteq \partial_t^2 - \partial_x^2 + 4q_k e^{-2 q_k x}V_k(x).
\end{equation*}
A direct computation yields that $\psi_c$ obeys (\ref{eq:forcedeqn1}) with right hand side
\begin{align}
    f(t,x) &= \mathcal{T}_k(\chi \psi) - 4q_k e^{-2q_k x}\chi \mathcal{E}_{p,0}(t,x) \nonumber \\
    &= \underbrace{[\mathcal{T}_k, \chi]\psi}_{g_0(t,x)} - \underbrace{4q_k e^{-2q_k x}\chi \mathcal{E}_{p,0}(t,x)}_{g_1(t,x)}. \label{eq:forcingtemp}
\end{align}
The forcing decomposes as a sum $g_0(t,x) + g_1(t,x)$, with the former compactly supported in $t$, and the latter rapidly decaying in $t$ by assumption on the background spacetime (cf. Definition \ref{dfn:admissiblespacetimesDEFN}). In particular, the assumptions (\ref{52:forcingassTOTAL}) hold for some constant $C$, and an index $\beta = \alpha > p_k$. 

Fix a constant $\beta_*' \in (1, \beta_*)$. By Proposition \ref{prop:resonanceexp}, there exists a constant $c_{\infty}^{(0)}$ independent of $x_0$ such that for all $\{x \leq x_0, t \geq 2 \}$ we have\footnote{Note we may replace $r_k$ with $r$ in (\ref{eq:resonanceexp}), by the assumed rapid decay of ${r - r_k}$.}
\begin{equation}
    \label{eq:completingprooftemp1}
    r(t,x) \big(\varphi(t,x) - c_{\infty}^{(0)}\big)= e^{-\beta_*' t}\mathcal{E}_{x_0}(t,x),
\end{equation}
for an error $\mathcal{E}_{x_0}(t,x)$ satisfying
\begin{equation}
    \label{eq:completingprooftemp2}
   \sup_{\{t \geq 1 \}} \| \mathcal{E}_{x_0}(t,x) \|_{C^2_{x}([0,x_0])} \leq C e^{\beta_*' x_0}
\end{equation}
uniformly in $x_0$, where $C$ depends on the $C^{\alpha}_{(hor)}$ norm of initial data, but not on $x_0$. 

\vspace{.5em}
\underline{Near-axis decay}: \
We next understand the implications of the decay (\ref{eq:completingprooftemp1})--(\ref{eq:completingprooftemp2}) in similarity coordinates. For fixed $z_0 \in (-1,0)$, define the near-axis region $\mathcal{S}_{z_0}$ and near-horizon region $\mathcal{D}_{z_0}$
\begin{align*}
    \mathcal{S}_{z_0} \doteq \{s \geq 2, -1 \leq z \leq z_0 \}, \quad \mathcal{D}_{z_0} \doteq \{s \geq 2, z_0 \leq z \leq 0\}.
\end{align*}
Defining $x_0 \doteq -\frac{1}{2q_k}\ln |z_0|$, we have $\mathcal{S}_{z_0} \subset \{t \geq 2, x \leq x_0 \}$, and from (\ref{eq:completingprooftemp1})--(\ref{eq:completingprooftemp2}), the averaging estimate (\ref{eq:averagingest}), as well as direct integration of (\ref{eq:wavesim}) we conclude
\begin{equation}
    \label{eq:completingprooftemp_est1}
    \|e^{\beta_*' s} r\big(\varphi - c_{\infty}^{(0)}\big)  \|_{C^2_{s,z}(\mathcal{S}_{z_0})} + \|e^{(\beta_*'-1) s} \varphi \|_{C^1_{s,z}(\mathcal{S}_{z_0})} \leq_{z_0} C.
\end{equation}
The main tool in propagating control to $\mathcal{D}_{z_0}$ will be multiplier estimates. There is, however, an estimate we may already close on $\varphi$. To see this, compute $e^{\beta_*' x} e^{-\beta_*' t} = e^{-\beta_*' s}$, and thus we can estimate (\ref{eq:completingprooftemp1})--(\ref{eq:completingprooftemp2}) in $L^\infty_{(\{s=\text{const}.\})}$, with no adverse dependence on $x_0$. It follows that 
\begin{equation}
    \label{eq:completingprooftemp_est2}
    \|e^{\beta_*' s} r\big(\varphi - c_{\infty}^{(0)}\big) \|_{L^{\infty}(\mathcal{D}_{z_0}) } \leq C.
\end{equation} 

\vspace{.5em}
\underline{Near-horizon decay}: \
We are now in a position to apply our multiplier estimates. Let $\rho \in (1-\beta_*', -k^2)$, and define $\psi_\rho \doteq e^{(q_k-\rho)s}r (\varphi - c_\infty^{(0)})$, which satisfies the (commuted) equation (\ref{eq:wavesim_alpha_comm0}). We repeat a form of this equation here for convenience:
\begin{equation}
    \label{eq:wavesim_alpha_comm0_rewritten}
    \partial_s \partial_z^2 \psi_\rho - q_k |z| \partial_z^3 \psi_\rho + (q_k + \rho)\partial_z^2 \psi_\rho + V \partial_z \psi_\rho + V' \psi_\rho = 0.
\end{equation}
Let $\omega = 0$ if $\alpha \geq \frac32$, and $\omega = \frac32 - \alpha + \epsilon$ if $p_k < \alpha \leq \frac32$, where $\epsilon \ll 1$ is sufficiently small. In the former case, it is straightforward to see that the multiplier estimate (\ref{eq:energyest2_0}) closes---we have concluded an estimate for $\|\partial_z \psi_\rho\|_{L^2_s(\Gamma_{s_0})}$, which concerns decay only in $\mathcal{S}_{z_0}$. Moreover, the coefficient of the bulk term can be made non-negative for $\rho$ sufficiently small, but \textit{strictly less}\footnote{Recall that $\rho = -k^2$ corresponds to $\psi \sim e^{-s},$ which is precisely the self-similar rate. Showing faster than self-similar decay requires establishing bounds for some $\rho < -k^2$. } than $-k^2$. It follows that in this case, we have the control
\begin{equation}
    \label{eq:completingprooftemp_est3}
    \sup_{\{s' \geq 0 \}}\|\partial_z^2 \psi_\rho \|_{L^2(\{s=s'\})} \leq C, \quad (\alpha \geq \frac32).
 \end{equation}
We wish to establish a similar form of (\ref{eq:completingprooftemp_est3}) in the lower regularity setting with $p_k < \alpha \leq \frac32$. The above argument does not apply to $\alpha \approx p_k$, as one can no longer guarantee that the bulk term in (\ref{eq:energyest2_0}) has a good sign.

However, we proceed by an analogous multiplier estimate, exploiting the additional control (\ref{eq:completingprooftemp_est1})--(\ref{eq:completingprooftemp_est2}). Multiplying (\ref{eq:wavesim_alpha_comm0_rewritten}) by $|z|^{2\omega}\partial_z^2 \psi_\rho$ and integrating by parts in $\mathcal{R}(s_0)$ yields (compare with (\ref{eq:temp2ndordermultiplier}))
\begin{align}
        \int_{\{s=s_0\}}&|z|^{2\omega}(\partial_z^2\psi_\rho)^2 dz + (q_k(1-2\omega)+2\rho)\iint_{\mathcal{R}(s_0)} |z|^{2\omega}(\partial_z^2 \psi_\rho)^2 dsdz \nonumber  \\[\jot]
        &\leq \int_{\{s=0\}}|z|^{2\omega}(\partial_z^2\psi_\rho)^2 dz - \underbrace{\iint_{\mathcal{R}(s_0)} 2 V |z|^{2\omega}\partial_z \psi_\rho \partial_z^2 \psi_\rho dzds}_{\text{I}} - \underbrace{\iint_{\mathcal{R}(s_0)} 2 V' |z|^{2\omega}\psi_\rho \partial_z^2 \psi_\rho dzds}_{\text{II}} . \label{eq:completingprooftemp2.5}
\end{align}
As $\alpha > p_k$, one can choose $\rho < -k^2$ and $\epsilon \ll 1$ such that the bulk term on the left hand side of the estimate is positive. For the term $\text{I}$, integrate by parts in $z$ to give
\begin{align}
    \text{I} &= - \int_{\Gamma_{s_0}} V (\partial_z \psi_p)^2 ds - \iint_{\mathcal{R}(s_0)} \partial_z \big(V |z|^{2\omega}  \big) (\partial_z \psi_p)^2 dzds \nonumber \\[\jot]
    &= - \int_{\Gamma_{s_0}} V (\partial_z \psi_p)^2 ds - \iint_{\{z \leq z_k \}} \partial_z \big(V |z|^{2\omega}  \big) (\partial_z \psi_p)^2 dzds - \iint_{\{z \geq z_k \}} \partial_z \big(V |z|^{2\omega}  \big) (\partial_z \psi_p)^2 dzds, \label{eq:completingprooftemp3}
\end{align}
where $z_k$ is the value defined in Proposition \ref{lem:propertiesofV}. From the repulsivity estimate (\ref{eq:potentialest_repulsivity}), it follows that the only term in (\ref{eq:completingprooftemp3}) which is supported near the horizon has a good sign! The remaining terms are supported near the axis, and are controlled by (\ref{eq:completingprooftemp_est1}).

For $\text{II}$ we exploit that by our choice of $\rho$ and (\ref{eq:completingprooftemp_est2}), there exists a $\delta \ll 1$ sufficiently small and constant $C$ such that 
\begin{equation}
    \| e^{\delta s}\psi_{\rho} \|_{L^2_{s,z}(\mathcal{R}(s_0))} \leq C.
\end{equation}
Therefore, for a small constant $\epsilon$
\begin{align*}
    |\text{II}| & \lesssim \epsilon  \iint_{\mathcal{R}(s_0)} e^{-2\delta s} |z|^{2\omega} (\partial_z^2 \psi_p)^2 dzds +  \epsilon^{-1} \iint_{\mathcal{R}(s_0)} e^{-2\delta s} |z|^{2\omega} \psi_p^2 dzds \\[\jot]
    &\lesssim \epsilon \sup_{s' \in [0,s_0]} \int_{\{s=s' \}} |z|^{2\omega} (\partial_z^2 \psi_p )^2 dz + C \epsilon^{-1}.
\end{align*}
Revisiting (\ref{eq:completingprooftemp2.5}), taking supremum over $s' \in [0,s_0]$, absorbing the contribution of term $\text{II}$, and applying the control (\ref{eq:completingprooftemp_est1})--(\ref{eq:completingprooftemp_est2}) to estimate the remaining terms supported near the axis, we ultimately conclude
\begin{equation}
    \label{eq:completingprooftemp_est4}
    \sup_{\{s' \geq 0 \}} \||z|^{\omega}\partial_z^2 \psi_\rho \|_{L^2(\{s=s'\})} \leq C, \quad (\alpha \leq \frac32),
 \end{equation}
 for some ${\rho < -k^2}$. Pointwise bounds on $\partial_z \varphi$ in $\mathcal{D}_{z_0}$ now follow by integrating (\ref{eq:completingprooftemp_est3}), (\ref{eq:completingprooftemp_est4}), and using the control in $\mathcal{S}_{z_0}$. Similarly, $\partial_s \varphi$ is estimated by integrating (\ref{eq:wavesim}) in $z$ from the axis. After translating to double-null coordinates, we conclude the proof.



\subsubsection*{Theorem \ref{theorem:mainthm}(b)}
We now turn to the case of threshold initial data $(r\varphi)_0(v) \in \mathcal{C}^{p_k k^2, \delta}_{(hor)}([-1,0])$, $\delta > 0$. As above, let $\psi(u,v) = (r\varphi)(u,v)$ denote the associated solution to (\ref{sec2.5:eq2}) in $\{u \geq -1\}$. 

The key observation is Lemma \ref{lem:holderspacedecomp}, asserting that general threshold data splits as the union of a one-dimensional subspace (spanned by $\mr{\phi}(z)$) and spaces of strictly higher regularity. In particular, there exists a constant $c_0$ such that $\varphi_0(z) - c_0 \mr{\phi}(z) \in \mathcal{C}^{p_k k^2 + \delta'}_{(hor)}([-1,0])$, for a $0 < \delta' \ll 1$ sufficiently small. By linearity and Theorem \ref{theorem:mainthm}(a), it suffices to assume $\varphi_0(z) = \mr{\phi}(z)$.

Define $\tilde{\psi}(s,z) \doteq (r \varphi)(s,z) - (r_k \phi_k)(s,z)$. 







\subsubsection*{Theorem \ref{theorem:mainthm}(c)}

\subsection{Proof of Theorem \ref{theorem:angularthm}}
\label{subsec:proofcompleted_4}


















==> temp_storage <==
Intuitively, one may expect this argument to apply in the case of interior perturbations as well. Although the integrand in (\ref{eq:intro2}) is now itself a dynamical quantity, it is still the case that unless a cancellation occurs between the two terms in (\ref{eq:intro2}), the conclusion of the previous paragraph should hold. 

\vspace{1em}
    \noindent
    \textbf{Stable singularity formation for nonlinear wave equations: } 
    The phenomenon of singularity formation via self-similar concentration, or more generally the concentration of a stationary profile, is ubiquitous in the study of hyperbolic equations---see examples for the wave maps equation \cite{IgorSterb, kriegerschlagtat_WM}, Yang-Mills \cite{kriegerschlagtat_YM}, and wave equations with power nonlinearity \cite{kriegerschlagtat_NLW}.

    The dynamical relevance of these solutions is determined by their stability, itself closely related to spectral properties of a linearized operator \cite{donninger2023} in appropriate function spaces. Establishing (finite codimension) mode-stability for these operators is a significant hurdle, often requiring equation-specific techniques and/or high degrees of smoothness. In many studies of stability \cite{burzio_krieger, kriegermiao, kriegermiaoschlag}, the background solutions have finite regularity, further complicating the analysis.

    A similar interpretation applies to the analysis of Section \ref{sec:scattering}. The $k$-self-similar spacetimes are finite regularity, singularity forming solutions to the Einstein-scalar field system, and the main result of Section \ref{sec:scattering} is a proof of mode stability for a family $P_k(\sigma)$ of operators arising from (\ref{eq:1}). The tractability of the problem in our setting is due to the relatively simple form of $P_k(\sigma)$ for $k$ sufficiently small.
